Hyperspectral Image Super-Resolution in Arbitrary Input-Output Band Settings

Hyperspectral image (HSI) with narrow spectral bands can capture rich spectral information, but it sacrifices its spatial resolution in the process. Many machine-learning-based HSI super-resolution (SR) algorithms have been proposed recently. However, one of the fundamental limitations of these approaches is that they are highly dependent on image and camera settings and can only learn to map an input HSI with one specific setting to an output HSI with another. However, different cameras capture images with different spectral response functions and bands numbers due to the diversity of HSI cameras. Consequently, the existing machine-learning-based approaches fail to learn to super-resolve HSIs for a wide variety of input-output band settings. We propose a single Meta-Learning-Based Super-Resolution (MLSR) model, which can take in HSI images at an arbitrary number of input bands' peak wavelengths and generate SR HSIs with an arbitrary number of output bands' peak wavelengths. We leverage NTIRE2020 and ICVL datasets to train and validate the performance of the MLSR model. The results show that the single proposed model can successfully generate super-resolved HSI bands at arbitrary input-output band settings. The results are better or at least comparable to baselines that are separately trained on a specific input-output band setting.

==> parts/comparison-vis.tex <==
\begin{figure*}[t]
\captionsetup{font={footnotesize}}
\centering
\begin{minipage}[t]{\textwidth}
% \vspace{0pt}
% \vspace*{\fill}
\centering
\setlength{\tabcolsep}{5pt}
\renewcommand{\arraystretch}{0}
\begin{tabular}[c]{cccc}
   \begin{subfigure}[c]{0.23\textwidth}
      \includegraphics[width=\textwidth]{images/ntire_result/test.png}
      \vspace{-0.6cm}
      \caption*{HR}
      \label{fig:hr1}
    \end{subfigure}&
    \begin{subfigure}[c]{0.23\textwidth}
      \includegraphics[width=\textwidth]{images/ntire_result/test.png}
      \vspace{-0.6cm}
      \caption*{Linear+Bicubic}
      \label{fig:lr_roi1}
    \end{subfigure}&
    \begin{subfigure}[c]{0.23\textwidth}
      \includegraphics[width=\textwidth]{images/ntire_result/test.png}
      \vspace{-0.6cm}
      \caption*{Linear+EDSR}
      \label{fig:sepedvr1}
    \end{subfigure}&
    \begin{subfigure}[c]{0.23\textwidth}
      \includegraphics[width=\textwidth]{images/ntire_result/test.png}
      \vspace{-0.6cm}
      \caption*{Linear+RDN}
      \label{fig:dainrbpn1}
    \end{subfigure}&
    \begin{subfigure}[c]{0.23\textwidth}
      \includegraphics[width=\textwidth]{images/ntire_result/test.png}
      \vspace{-0.6cm}
      \caption*{Cubic+Bicubic}
      \label{fig:adarbpn1}
    \end{subfigure}&
    \begin{subfigure}[c]{0.23\textwidth}
      \includegraphics[width=\textwidth]{images/ntire_result/test.png}
      \vspace{-0.6cm}
      \caption*{Cubic+EDSR}
      \label{fig:adaedvr1}
    \end{subfigure}&
    \begin{subfigure}[c]{0.23\textwidth}
      \includegraphics[width=\textwidth]{images/ntire_result/test.png}
      \vspace{-0.6cm}
      \caption*{Cubic+RDN}
      \label{fig:dainedvr1}
    \end{subfigure}&
    \begin{subfigure}[c]{0.23\textwidth}
      \includegraphics[width=\textwidth]{images/ntire_result/test.png}
      \vspace{-0.6cm}
      \caption*{MLSR}
      \label{fig:}
    \end{subfigure}
    \end{tabular}
  \end{minipage}
  \caption{}
\label{fig:NITER_results}
\end{figure*}

==> parts/datasets_table.tex <==
\begin{table}[ht]
    \centering
    \begin{tabular}{l c c c}
    \thickhline
        Name & \makecell{Number\\of Images} & \makecell{Number\\of Bands} & \makecell{Range of\\wavelength}\\
        \hline
        \hline
        Painting\cite{zacharopoulosMethodRegistrationSpectral2018a} & 5 & 23 & 360-1150nm\\
        \hline
        UEA\cite{hordleyMultispectralImageDatabase2004} & 23 & 31 & 400-700nm\\
        \hline
        % Bristol\cite{parragaColorLuminanceInformation1998} & 29 & 31 & 400-700nm\\
        % \hline
        Foster\cite{nascimentoSpatialDistributionsLocal2016} & 30 & 33 & 400-720nm\\
        \hline
        CAVE\cite{yasumaGeneralizedAssortedPixel2010} & 32 & 31 & 400-700nm\\
        \hline
        Harvard\cite{chakrabartiStatisticsRealworldHyperspectral2011} & 52 & 31 & 420-720nm\\
        \hline
        ICVL\cite{aradSparseRecoveryHyperspectral2016a} & 201 & 31 & 400-700nm\\
        \hline
        NTIRE2020\cite{aradNTIRE2020Challenge2020} & 460 & 31 & 400-700nm\\
    \thickhline
    \end{tabular}
    \caption{Summary of publicly available HSI Datasets.}
    \label{tab:datasets}
\end{table}


% \begin{table}[ht]
%     \centering
%     \begin{tabular}{l c c c c}
%     \thickhline
%         Name & \makecell{Number\\of Images} & \makecell{Number\\of Bands} & \makecell{Range of\\wavelength} & Steps \\
%         \hline
%         \hline
%         \href{https://projects.ics.forth.gr/cvrl/msi/}{Painting} & 5 & 23 & 360-1150nm & Unfixed\\
%         \hline
%         \href{http://colour.cmp.uea.ac.uk/datasets/multispectral.html}{UAE} & 23 & 31 & 400-700nm & 10nm\\
%         \hline
%         \href{http://www.cvc.uab.es/color_calibration/Bristol_Hyper/}{Bristol} & 29 & 31 & 400-700nm & 10nm\\
%         \hline
%         \href{https://personalpages.manchester.ac.uk/staff/d.h.foster/Local_Illumination_HSIs/Local_Illumination_HSIs_2015.html}{Foster} & 30 & 33 & 400-720nm & 10nm\\
%         \hline
%         \href{https://www.cs.columbia.edu/CAVE/databases/multispectral/}{CAVE} & 32 & 31 & 400-700nm & 10nm\\
%         \hline
%         \href{http://vision.seas.harvard.edu/hyperspec/explore.html}{Harvard} & 52 & 31 & 420-720nm & 10nm\\
%         \hline
%         \href{http://icvl.cs.bgu.ac.il/hyperspectral/}{ICVL} & 201 & 31 & 400-700nm & 10nm\\
%         \hline
%         \href{https://competitions.codalab.org/competitions/22225#participate}{NTIRE2020} & 460 & 31 & 400-700nm & 10nm\\
%     \thickhline
%     \end{tabular}
%     \caption{Summary of publicly available HSI Datasets.}
%     \label{tab:datasets}
% \end{table}

==> parts/inbands_psnr.tex <==
\begin{figure}[t]
% \captionsetup{font={footnotesize}}
\centering
% \vspace{0pt}
% \vspace*{\fill}
\centering
    \includegraphics[width=\columnwidth]{images/inbands-psnr/5-bands_mean_methods_psnr.png}
    \caption{Illustration of performance comparison on different methods given the same input bands number(5 bands here). The gray vertical dash lines mean the HSI band at that index is included the LR HSI input.}
\label{fig:inbands_psnr}
\end{figure}



% \begin{figure*}[t]
% \captionsetup{font={footnotesize}}
% \centering
% \begin{minipage}[t]{\textwidth}
% % \vspace{0pt}
% % \vspace*{\fill}
% \centering
% \setlength{\tabcolsep}{0pt}
% \renewcommand{\arraystretch}{0}
% \begin{tabular}[c]{ccc}
% \multirow{2}{*}[41pt]{
%     \begin{subfigure}{0.52\textwidth}
%       \includegraphics[width=\textwidth]{images/inbands-psnr/5-bands_mean_methods_psnr.png}
%       \vspace{-0.8cm}
%       \caption*{(a) 5-bands}
%       \label{fig:SSSR}
%     \end{subfigure}
% }&
%   \begin{subfigure}[c]{0.23\textwidth}
%       \includegraphics[width=\textwidth]{images/inbands-psnr/6-bands_mean_methods_psnr.png}
%       \vspace{-0.6cm}
%       \caption*{(b) 6-bands}
%       \label{fig:c_b}
%     \end{subfigure}&
%     \begin{subfigure}[c]{0.23\textwidth}
%       \includegraphics[width=\textwidth]{images/inbands-psnr/7-bands_mean_methods_psnr.png}
%       \vspace{-0.6cm}
%       \caption*{(c) 7-bands}
%       \label{fig:c_e}
%     \end{subfigure}\\&
%     \begin{subfigure}[c]{0.23\textwidth}
%       \includegraphics[width=\textwidth]{images/inbands-psnr/8-bands_mean_methods_psnr.png}
%       \vspace{-0.6cm}
%       \caption*{(d) 8-bands}
%       \label{fig:c_r}
%     \end{subfigure}&
%     \begin{subfigure}[c]{0.23\textwidth}
%       \includegraphics[width=\textwidth]{images/inbands-psnr/9-bands_mean_methods_psnr.png}
%       \vspace{-0.6cm}
%       \caption*{(e) 9-bands}
%       \label{fig:l_b}
%     \end{subfigure}
%     \end{tabular}
%   \end{minipage}
%   \caption{Illustration of performance comparison on different methods given the same input bands number. The gray vertical dash lines mean input HSI contain band at that index.}
% \label{fig:inbands_psnr}
% \end{figure*}

==> parts/methods_psnr.tex <==
\begin{figure}[t]
% \captionsetup{font={footnotesize}}
\centering
\begin{minipage}[t]{\columnwidth}
% \vspace{0pt}
% \vspace*{\fill}
\centering
\setlength{\tabcolsep}{0pt}
\renewcommand{\arraystretch}{0}
\begin{tabular}[c]{cc}
    \begin{subfigure}[c]{\columnwidth}
      \includegraphics[width=\columnwidth]{images/methods-psnr/c_r_mean_inbands_psnr.png}
      \vspace{-0.7cm}
      \caption*{(c) Cubic+RDN}
      \label{fig:c_e}
    \end{subfigure}\\
    \begin{subfigure}[c]{\columnwidth}
      \includegraphics[width=\columnwidth]{images/methods-psnr/sssr_mean_inbands_psnr.png}
      \vspace{-0.7cm}
      \caption*{(d) MLSR}
      \label{fig:c_r}
    \end{subfigure}
    \end{tabular}
  \end{minipage}
  \caption{Illustration of performance comparison on different input band number for MLSR and two baseline methods. The small triangles pointing down mean input HSI contains this band. Triangles with different colors is corresponding to the curve of the same color.}
\label{fig:methods_psnr}
\end{figure}










% \begin{figure}[t]
% \captionsetup{font={footnotesize}}
% \centering
% \begin{minipage}[t]{\columnwidth}
% % \vspace{0pt}
% % \vspace*{\fill}
% \centering
% \setlength{\tabcolsep}{0pt}
% \renewcommand{\arraystretch}{0}
% \begin{tabular}[c]{cc}
% \multirow{2}{*}[38pt]{
%     \begin{subfigure}{0.6\columnwidth}
%       \includegraphics[width=\columnwidth]{images/methods-psnr/sssr_mean_inbands_psnr.png}
%       \vspace{-0.3cm}
%       \caption*{(a) MLSR}
%       \label{fig:SSSR}
%     \end{subfigure}}&
%     \begin{subfigure}[c]{0.37\columnwidth}
%       \includegraphics[width=\columnwidth]{images/methods-psnr/c_e_mean_inbands_psnr.png}
%       \vspace{-0.7cm}
%       \caption*{(c) Cubic+EDSR}
%       \label{fig:c_e}
%     \end{subfigure}\\&
%     \begin{subfigure}[c]{0.37\columnwidth}
%       \includegraphics[width=\columnwidth]{images/methods-psnr/c_r_mean_inbands_psnr.png}
%       \vspace{-0.7cm}
%       \caption*{(d) Cubic+RDN}
%       \label{fig:c_r}
%     \end{subfigure}
%     \end{tabular}
%   \end{minipage}
%   \caption{Illustration of performance comparison on different input bands number for MLSR and two baseline methods. The small triangles pointing down mean input HSI contains this band. Triangles with different colors is corresponding to the curve of the same color.}
% \label{fig:methods_psnr}
% \end{figure}






% \begin{figure*}[t]
% \captionsetup{font={footnotesize}}
% \centering
% \begin{minipage}[t]{\textwidth}
% % \vspace{0pt}
% % \vspace*{\fill}
% \centering
% \setlength{\tabcolsep}{0pt}
% \renewcommand{\arraystretch}{0}
% \begin{tabular}[c]{cccc}
% \multirow{2}{*}[41pt]{
%     \begin{subfigure}{0.42\textwidth}
%       \includegraphics[width=\textwidth]{images/methods-psnr/fasr_mean_inbands_psnr.png}
%       \vspace{-0.8cm}
%       \caption*{(a) MLSR}
%       \label{fig:SSSR}
%     \end{subfigure}
% }&
%   \begin{subfigure}[c]{0.19\textwidth}
%       \includegraphics[width=\textwidth]{images/methods-psnr/c_b_mean_inbands_psnr.png}
%       \vspace{-0.6cm}
%       \caption*{(b) Cubic+Bicubic}
%       \label{fig:c_b}
%     \end{subfigure}&
%     \begin{subfigure}[c]{0.19\textwidth}
%       \includegraphics[width=\textwidth]{images/methods-psnr/c_e_mean_inbands_psnr.png}
%       \vspace{-0.6cm}
%       \caption*{(c) Cubic+EDSR}
%       \label{fig:c_e}
%     \end{subfigure}&
%     \begin{subfigure}[c]{0.19\textwidth}
%       \includegraphics[width=\textwidth]{images/methods-psnr/c_r_mean_inbands_psnr.png}
%       \vspace{-0.6cm}
%       \caption*{(d) Cubic+RDN}
%       \label{fig:c_r}
%     \end{subfigure}\\&
%     \begin{subfigure}[c]{0.19\textwidth}
%       \includegraphics[width=\textwidth]{images/methods-psnr/l_b_mean_inbands_psnr.png}
%       \vspace{-0.6cm}
%       \caption*{(e) Linear+Bicubic}
%       \label{fig:l_b}
%     \end{subfigure}&
%     \begin{subfigure}[c]{0.19\textwidth}
%       \includegraphics[width=\textwidth]{images/methods-psnr/l_e_mean_inbands_psnr.png}
%       \vspace{-0.6cm}
%       \caption*{(f) Linear+EDSR}
%       \label{fig:l_e}
%     \end{subfigure}&
%     \begin{subfigure}[c]{0.19\textwidth}
%       \includegraphics[width=\textwidth]{images/methods-psnr/l_r_mean_inbands_psnr.png}
%       \vspace{-0.6cm}
%       \caption*{(g) Linear+RDN}
%       \label{fig:l_r}
%     \end{subfigure}
%     \end{tabular}
%   \end{minipage}
%   \caption{Illustration of performance comparison on different input bands number for MLSR and all other baseline methods. The small triangles pointing down mean input HSI contains this band. Triangles with different colors is corresponding to the curve of the same color.}
% \label{fig:methods_psnr}
% \end{figure*
